Hard negative examples are hard, but useful

Triplet loss is an extremely common approach to distance metric learning. Representations of images from the same class are optimized to be mapped closer together in an embedding space than representations of images from different classes. Much work on triplet losses focuses on selecting the most useful triplets of images to consider, with strategies that select dissimilar examples from the same class or similar examples from different classes. The consensus of previous research is that optimizing with the \textit{hardest} negative examples leads to bad training behavior. That's a problem -- these hardest negatives are literally the cases where the distance metric fails to capture semantic similarity. In this paper, we characterize the space of triplets and derive why hard negatives make triplet loss training fail. We offer a simple fix to the loss function and show that, with this fix, optimizing with hard negative examples becomes feasible. This leads to more generalizable features, and image retrieval results that outperform state of the art for datasets with high intra-class variance.

==> table/CUBCAR.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{0.2em}
\begin{center}
\begin{tabular}{|c|cccc|cccc|}
\hline
Dataset & 
\multicolumn{4}{|c|}{CUB} & \multicolumn{4}{|c|}{CAR}\\
\hline
Method & R@1 & R@2 & R@4 & R@8 & R@1 & R@2 & R@4 & R@8\\
\hline
Triplet-Semihard$^{64}$(GoogleNet)
& 42.6 & 55.03 & 66.4 & 77.2
& 51.5 & 63.8 & 73.5 & 82.4\\
Lifted$^{64}$(GoogleNet)
& 43.6 & 56.6 & 68.6 & 79.6
& 53.0 & 65.7 & 76.0 & 84.3\\
Clustering$^{64}$(GoogleNet)
& 49.8 & 61.4 & 71.8 & 81.9
& 58.1 & 70.6 & 80.3 & 87.8\\
SmartMining$^{64}$(GoogleNet)
& 49.8 & 62.3 & 74.1 & 83.3
& 64.7 & 76.2 & 84.2 & 90.2\\
ProxyNCA$^{64}$(GoogleNet)
& 49.2 & 61.9 & 67.9 & 72.4
& 73.2 & 82.4 & 86.4 & 88.7\\ 
N-pair$^{64}$(GoogleNet)
& 51.9 & 64.3 & 74.9 & 83.2
& 71.1 & 79.7 & 86.5 & 91.6\\
Multi-Similarity$^{64}$(InceptionBN)
& 57.4 & 69.8 & 80.0 & {\bf 87.8}
& 77.3 & 85.3 & 90.5 & 94.2\\
EasyPositive(EPSHN)$^{64}$(ResNet50)
& 57.3 & 68.9 & 79.3 & 87.2
& 75.5 & 84.2 & 90.3 & 94.2\\
OURS(EPHN)$^{64}$(GoogleNet)
& 58.8 & 70.2 & 78.9 & 86.8
& 76.7 & 84.5 & 90.4 & 94.3\\
OURS(EPHN)$^{64}$(ResNet50)
& {\bf 60.0} & {\bf 71.0} & {\bf 80.5} & 87.6
& {\bf 80.0} & {\bf 87.1} & {\bf 91.4} & {\bf 94.8} \\
\hline
\end{tabular}
\end{center}
\caption{Retrieval Performance on the CUB and CAR datasets comparing to the best reported results for more approaches with embedding dimension 64.}
\label{table:CUBCAR}
\end{table*}


==> table/Hotel_2nd.tex <==
\begin{table}[t]
\begin{center}
\begin{tabular}{|c|ccc|}
\hline
Dataset & \multicolumn{3}{|c|}{Hotel Instance}  \\

\hline
Method & R@1 & R@10 & R@100 \\
\hline
BATCH-ALL~\cite{hotels50k}$^{256}$ & 8.1 & 17.6 & 34.8 \\
Easy Positive(EPSHN)~\cite{xuan2019improved}$^{256}$ & 16.3 & 30.5 & 49.9 \\
\hline
OURS(EPHN)$^{256}$ & \bf{21.1} & \bf{34.5} & \bf{50.6} \\
\hline
\end{tabular}
\end{center}
\caption{Retrieval performance on the Hotels-50K dataset. All methods are trained with Resnet-50 and embedding size is 256.}
\label{table:Hotels}
\end{table}

==> table/SOPICR_2nd.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{0.2em}
\begin{center}
\begin{tabular}{|c|ccc|ccc|}
\hline
Dataset & 
\multicolumn{3}{|c|}{SOP} & \multicolumn{3}{|c|}{In-shop}\\
\hline
Method & R@1 & R@10 & R@100& R@1 & R@10 & R@20\\
\hline
BIER~\cite{BIER}$^{512}$
& 72.7 & 86.5 & 94.0 
& 76.9 & 92.8 & 95.2 \\
ABE~\cite{ABE}$^{512}$
& 76.3 & 88.4 & 94.8 
& 87.3 & 96.7 & 97.9 \\
FastAP~\cite{Cakir_2019_CVPR}$^{512}$
& 76.4 & 89.0 & 95.1
& \bf{90.9} & \bf{97.7} & \bf{98.5}\\
MS~\cite{wang2019multi}$^{512}$ 
& 78.2 & 90.5 & 96.0
& 89.7 & 97.9 & 98.5\\
EasyPositive(EPSHN)~\cite{xuan2019improved}$^{512}$ 
& 78.3 & 90.7 & 96.3
& 87.8 & 95.7 & 96.8\\
\hline
OURS(EPHN)$^{512}$ 
& \bf{80.8} & \bf{92.3} & \bf{96.7}
& 90.5 & 97.5 & 98.2\\
\hline
\end{tabular}
\end{center}
\caption{Retrieval Performance on the SOP and In-shop datasets comparing to the best reported results for more complex approaches and/or ensembles. Test is trained with ResNet50}
\label{table:SOPICR}
\end{table*}

==> table/datasets.tex <==
\begin{table*}[t]
\setlength{\tabcolsep}{0.2em}
\begin{center}
\begin{tabular}{|c|ccc|ccc|ccc|ccc|}
\hline
Dataset & 
\multicolumn{3}{|c|}{CUB(n=8)} & \multicolumn{3}{|c|}{CAR(n=16)} & \multicolumn{3}{|c|}{SOP(n=2)} & \multicolumn{3}{|c|}{In-shop(n=2)}\\
\hline
Method & R@1 & R@2 & R@4 & R@1 & R@2 & R@4 & R@1 & R@10 & R@100& R@1 & R@10 & R@20\\
\hline
EPSHN(1st)
& 55.7 & 67.8 & 78.2
& 72.8 & 82.2 & 88.7
& 77.4 & 90.0 & 96.2
& 86.5 & 96.7 & 97.7 \\
EPSHN(2nd)
& 56.0 & 68.3 & 78.3
& 76.6 & 84.8 & 90.3
& 78.0 & 90.3 & 96.2
& 88.1 & 96.7 & 97.6 \\
EPHN(1st)
& 55.1 & 67.3 & 78.3
& 72.6 & 81.7 & 88.6
& 78.0 & 90.6 & 96.3
& 87.1 & 96.9 & 97.9 \\
EPHN(2nd)
& 57.1 & 68.9 & 79.2
& 77.8 & 85.4 & 90.3
& 78.8 & 90.8 & 96.3
& 89.0 & 96.9 & 97.8 \\
\hline
\end{tabular}
\end{center}
\caption{Retrieval Performance on the CUB, CAR, SOP and In-shop datasets with EPHN and EPSHN method. The CUB, CAR results are trained with ResNet18 and SOP and In-shop are trained with ResNet50}
\label{table:EPHN2EPSHN}
\end{table*}
